Chaos Engineering for Enhanced Resilience of Cyber-Physical Systems

Cyber-physical systems (CPS) incorporate the complex and large-scale engineered systems behind critical infrastructure operations, such as water distribution networks, energy delivery systems, healthcare services, manufacturing systems, and transportation networks. Industrial CPS in particular need to simultaneously satisfy requirements of available, secure, safe and reliable system operation against diverse threats, in an adaptive and sustainable way. These adverse events can be of accidental or malicious nature and may include natural disasters, hardware or software faults, cyberattacks, or even infrastructure design and implementation faults. They may drastically affect the results of CPS algorithms and mechanisms, and subsequently the operations of industrial control systems (ICS) deployed in those critical infrastructures. Such a demanding combination of properties and threats calls for resilience-enhancement methodologies and techniques, working in real-time operation. However, the analysis of CPS resilience is a difficult task as it involves evaluation of various interdependent layers with heterogeneous computing equipment, physical components, network technologies, and data analytics. In this paper, we apply the principles of chaos engineering (CE) to industrial CPS, in order to demonstrate the benefits of such practices on system resilience. The systemic uncertainty of adverse events can be tamed by applying runtime CE-based analyses to CPS in production, in order to predict environment changes and thus apply mitigation measures limiting the range and severity of the event, and minimizing its blast radius.

==> 1-introduction.tex <==
\section{Introduction} \label{Introduction}


%CPS and iCPS. The importance of resiliency against adverse events.
The term cyber-physical systems (CPS) refers to systems which integrate and interconnect the physical environment with control, computing, and networking components. In the last decade, there is a rapid growth of CPS in critical infrastructures including power systems, manufacturing facilities, robotics, transportation networks, desalination plants, and other industrial control systems (ICS). Due to the substantial applications of CPS, especially in industrial environments, their resilience (ability to  ``resist'' and ``recover'' from disrupting events) is of paramount importance for ensuring system reliability, quality, and security of operations \cite{9351954}. Adverse events including ‘silent errors’ due to components and manufacturing variability failures, hardware or software faults of smart monitoring devices due to bugs in the code (e.g., operating system, compilers, libraries, etc.), natural effects such as bit flips induced by hardware failures, drive failures, cosmic rays, cyber-attacks, faults involving the infrastructure design and implementation, or even natural disasters such as hurricanes, earthquakes, wildfires, pose significant threats to sustainable and resilient CPS and can lead to catastrophic impacts with financial, social, legal, and political impacts. 

%Experimentation practices to increase CPS resiliency: example HIL testbeds, digital twins. A more realistic approach which leverages the actual production environment as long as the event is constraint not to cause halt production is CE. Definition of CE.  

In order to enhance CPS resiliency, there exist various works on resilience definitions, metrics, and evaluation and enhancement methods. A conceptual resilience curve with resilient control metrics is the ``Disturbance and Impact Resilience Evaluation Curve'' (DIRE), presented in Fig. \ref{fig:dire}, that express the ``Rs'' of resilience, i.e., Recon, Resist, Respond, Recover, and Restore \cite{8088656}. Experimentation practices involve the use of hardware-in-the-loop (HIL) testbed environments \cite{9351954} and digital twins \cite{koulamas2018cyber}, Monte Carlo simulation-based methods \cite{yu2020resilient}, pre-selected scenario-based methods, and machine learning-based methods \cite{8255544}. 
Existing methods, however, are often not examined in deployed CPS nor governed by a proactive experimentation practice in which weaknesses can be revealed before impacting the system, e.g., often HIL experimentation is specific to the application and scenarios under test, and not following systematic experimentation steps. In this work, we present chaos engineering (CE) as an approach to enhance the resilience of CPS. CE has been primarily used for software systems, and can be defined as ``the discipline of experimenting on a system in order to build confidence in the system’s capability to withstand turbulent conditions in production'' \cite{miles2019learning}.


\begin{figure}
    \centering
    \includegraphics[width=0.95\columnwidth]{Figs/dire.png}
    %\vspace{-1mm}
    \caption{Disturbance and impact resilience evaluation (DIRE) Curve ($i$=initial, $f$=final) \cite{8088656}.}
    %\vspace{-6mm}
    \label{fig:dire}
\end{figure}


%CE details (netflix use) and benefits. See Emil's commented text below
CE involves the facilitation of experiments to reveal weaknesses within a system, i.e. how the system responds to unexpected events such as outages due to cyber-attacks or faults. The concept of CE was originated from Netflix in an effort to develop a built-in resilience tool within the production environment \cite{basiri2016chaos}. Typically, CE experiments include the following steps (Fig. \ref{fig:steps}): (1) define the `steady state' of a system in order to quantify its characteristic behavior under a certain type of events; (2) build a hypothesis around the steady state which should be followed in both the control/theoretical aspect and the experiments (measurable output of a system); (3) vary process events into the systems reflecting realistic adverse productions conditions; (4) run automated experiments within the system production environment in an effort to disprove the hypothesis in terms of control and experiments differences. This experimentation process builds confidence in the system with regards its steady states of operation and how hard they are to be disrupted. In case CE experimentation identifies a systemic weakness, the overall process is set up in a way to ensure that potential impact radius from the experiment is minimized and contained. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figs/steps.png}
     %\vspace{-5mm}
    \caption{Chaos engineering (CE) experimentation principles.}
     %\vspace{-4mm}
    \label{fig:steps}
\end{figure}

In terms of quantitative benefits, CE can reduce the number of preventable outages. This reduction of the blast radius is coupled with chaos-induced bounded harm that is revealed by CE experiments. 
Another aiding approach to CE is modeling outages using historical data, i.e. a proper implementation of CE experiments requires an establishment of a baseline for test metrics based on historical data. Taking proper records from an incident management system in place, and identifying vulnerabilities where the failure of a non-critical node could bring the system down leading to an outage, provides insight to quantitative financial loss due to the occurred incident as well as information about vulnerable nodes that should be injected in the next CE experiment. The adoption process may require engineers to mitigate risks of impacting customers with these experiments. This means there is a balance between reducing the impact to customers and identifying vulnerabilities quickly. As for qualitative benefits of CE, these include improvement in design decisions, growth in understanding service criticality, and confidence in validating reliability measures.


% In this paper, what we do.  + % Roadmap of the paper. 
In this paper, we introduce the concept of CE for enhancing the resilience of CPS, and specifically, ICS environments of critical infrastructures. First, we review experimentation practices for weaknesses identification and testing as well as present existing CE approaches (Section \ref{s:related}). We then build a case of a CE formal model in which we define and describe the control theoretical aspects of CE of a nonlinear cyber-physical ICS (Section \ref{s:model}). Furthermore, we present a use-case scenario on the industrial process control model of the Tennessee Eastman Challenge in an effort to map the CE experimentation steps with actual metrics and failure events (Section \ref{s:use-case}). 






\iffalse
Chaos engineering is a discipline that involves experimenting on a system to test the strengths or weaknesses within in a system. To further discuss, it gives the system operator a better idea of how the system will respond to unexpected events such as outages due to cyberattacks or weather, etc. Chaos engineering is very important since the complexity of the system in the ICS world is steadily increasing. To convince our readers of the benefits of Chaos Engineering, an implementation realized by Netflix can be shown. For the business side, making quantitative arguments based on historical data and presenting tangible benefits to the business, both are valid justifications of introduction of Chaos Engineering to the power grid~\cite{tucker2018business}.

Starting the list starts of quantitative benefits is a reduction in the number of preventable outages, meaning,  if chaos engineering is properly implemented, it is expected that fewer outages will occur. This reduction is coupled with chaos-induced harm that is revealed by chaos engineering experiment. In essence, chaos experiments uncover vulnerabilities in the system that otherwise have a potential to cause outages. To minimize harm induced during experiments, engineers reduce the blast radius by making it as small as possible while still being detectable. 
Another aiding approach to chaos engineering is modeling outages using historical data. Taking proper records from an incident management system in place, and identifying vulnerabilities where the failure of a non-critical node could bring the system down leading to an outage, provides insight to quantitative financial loss due to the occurred incident as well as information about vulnerable nodes that should be injected in the next chaos engineering experiment. 
Based two previous statements, a proper implementation of chaos engineering requires an establishment of a baseline for test metrics based on historical data. The adoption process may require engineers to mitigate risks of impacting customers with these experiments. This means there is a balance between reducing the impact to customers and identifying vulnerabilities quickly. 
Qualitative benefits of chaos engineering implementation are: an improvement in design decisions, growth in understanding service criticality, and confidence in validating reliability measures.

Chaos monkey was described as a software tool that aims to aid software engineers to design and implement services that are able to withstand failures of  individual instances ~\cite{bennett2012chaos}.

Another definition of chaos engineering with a proposed framework is given by ~\cite{jernberg2020building}. There, twelve open source chaos engineering tools are used with an aim to define and implement a continuous and extensible chaos engineering practice for a software system.
Aiding to the cause, another tool was constructed and presented in ~\cite{monge2020developing}. This tool greatly reduces the time taken by manual testing labor and aids software engineers to find potentially costly failures. The benefits of automation in chaos engineering are presented.

Several papers such as ~\cite{canonico2020human} introduce a human-AI partnerships for Chaos Engineering. According to authors, some aspects of AI would be used to make a system more resilient to perturbation and the results of these findings show improvement when compared to  existing chaos engineering approaches.

An exemplary successful implementation of chaos engineering is Netflix platform for automatically generating and executing chaos experiments~\cite{basiri2019automating}. Here we will give just a brief introduction to Netflix successful implementation of Chaos Engineering, to be later discussed in Section III as a very demonstrative example to then be connected with the CPS systems argument. 

\fi

==> 2-literature.tex <==

\section{Related Work and Limitations}\label{s:related} 

Modern distributed systems and content delivery networks are often implemented as software-based services. Testing and vulnerability detection in distributed systems is a broad field that borrows numerous techniques from different engineering fields. CPS, and in particular modern ICS are typically  implemented as distributed software-based systems that control embedded devices and field sensors, yet to our knowledge, there has been no prior use of CE experiments on ICS. As such, relevant publications cover two distinct areas, namely \textit{(A)} vulnerability detection and fault testing in ICS, and \textit{(B)} current practices of CE in distributed systems. 

\subsection {Vulnerability Detection and Fault Testing in ICS}

There exist several techniques for vulnerability detection and failure testing in software-based distributed systems that share common characteristics with CE experiments. In software, existing approaches can be broadly classified into: 
\begin{enumerate}

\item Static and Dynamic analysis methods including fuzzing techniques. These approaches identify issues inside the code of embedded components and industrial systems, either offline (static) or during run-time execution of software (dynamic).
\item Fault injection on ICS components, and 
\item Conditional testing approaches for the detection of system deviations, mostly implemented with invariant mining techniques.
\end{enumerate}

There is extensive research on static analysis of industrial software for fault detection. Recent approaches utilize various techniques, such as regression verification \cite{beckert2015regression}, model checking \cite{biallas2012arcade, canet2000towards}, or sequential function charts for the programming of the programmable logic controllers (PLCs). Similar approaches have extended these methods by including specifications of plant behavior converted to hybrid automata for verifying safety properties \cite{nellen2014cegar, nellen2016two}. 


Concerning dynamic analysis approaches, there exists %interesting 
work that delves into fault testing of ICS components. %Research work has presented various such implementations. 
Authors in \cite{guo2017symbolic} have presented how tools can generate test inputs through symbolic execution to detect program execution errors. VetPLC is another attempt that combines static and dynamic analysis presented in \cite{zhang2019towards}. Its goal is to verify real-world PLC code driven by events and detect safety violations in code. The work combines different types of analysis to understand causal relations among events in PLC code and quantitatively gauge temporal dependencies that are constrained by machine operations.

Published research has also uses fuzzy testing in ICS, with existing work targeting both industrial protocols and embedded systems. For example, authors in \cite{luo2019polar} were able to fuzzy test function codes in ICS protocols and extract semantic information for vulnerability detection. Other approaches opted to fuzz input commands on firmware binaries extracted from ICS to evaluate the security of specific libraries inside ICS components \cite{tychalas2020}. 

Mining invariant values from ICS devices has also been in scope of recent research in fault detection of ICS software. Recent approaches aim to extract operational conditions from system logs via data mining. These conditional variables are then evaluated whether they hold true at some point in time during varying executions of ICS processes  \cite{beschastnikh2011leveraging}, \cite{ohmann2014behavioral}. Other approaches  mine such conditions from smart meters and medical devices, mostly for intrusion detection purposes \cite{aliabadi2017artinali}. Chen \textit{et al.}  extracted invariants from data traces of a water purification test-bed to detect anomalies in system execution \cite{chen2018learning}. Other mixed approaches may also use invariants for vetting the source code of ICS components \cite{zhang2019towards}. 

CE experiments try to deal with the fact that functional charts and specifications cannot capture the scale and complexity of user behavior in modern distributed systems. As such, CE focuses on experimenting on the entire system under test as a single entity. Even though such approaches are not able to formally define function executions, they have shown great promise in uncovering unwanted states of execution that were previously unknown and not depicted in functional specifications \cite{basiri2016chaos, basiri2019automating}. CE experiments may also utilize fuzzing techniques for input, but they do not consider specific technical inputs or their fuzzed input does not target specific software or components. Instead, CE experiment view all ICS components and field devices as a single system and try to fuzz real-world, high-level input to observe what happens to the ICS boundary. 

Also, another difference between CE experiments and some of the aforementioned fault analysis and testing techniques lies on the fact that CE experiments do not follow a binary assertion logic (as is the case with invariants or static analysis). Most fault testing and assessment methods assign pre-considered restrictions and evaluate software-based systems against these precondition to assert them as true or false. Instead, CE experiments focus in creating new execution data and detect system states that were previously unknown to operators \cite{basiri2016chaos}.

\subsection{Existing CE Approaches}

Concerning existing CE experiments, the most famous case is Netflix, where engineers have taken CE as an approach to experimentally verify distributed systems' reliability. That is achieved either by changing the boundary state of components and analyzing system behavior using an internal service that was created specifically for his purpose (Chaos Monkey) \cite{basiri2016chaos}, or by introducing false injections at the boundary of Netflix micro-services \cite{basiri2019automating}. Chaos Monkey was also used in \cite{chang2015}, where researchers proposed a balanced use of the service to inject variable degrees of failure into the network without disconnecting it and assess it against network invariant metrics. 

Large-scale Java applications have also been known to utilize CE for testing complex distributed software \cite{zhang2019chaos}. Other implementations of the CE principles aimed to automatically inject system failures and errors into a containerized application to evaluate the overall system resilience under unknown states of operation \cite{simonsson2019}. Researchers in \cite{Przystalka2015} detected faults in industrial network data using recurrent neural networks that incorporate CE principles to improve the efficiency of the tuning procedure. Neural networks and CE was also proposed in \cite{aihara2002chaos} as a means for generating unwanted states in nonlinear electrical circuits. Authors aimed to discover vulnerabilities on large, complex systems, such as the U.S. power grid. 

Other research has focused on using CE for analyzing the execution states of Infrastructure-as-a-Service (IaaS) cloud platforms. For example, CloudStrike implemented the principles of CE by injecting faults to cloud resources to experiment on cybersecurity breaches caused by human errors and misconfigured resources  \cite{torkura2019security, torkura2020CloudStrike}. 

==> 3-cemodel.tex <==
\section{A Generic Chaos Engineering (CE) Model}\label{s:model}

The cyber-physical model of ICS can be seen as a model of a nonlinear system in the following state-space form: 
\begin{align}
\dot{x}(t) &=g(x(t), u(t), \delta(t)) \label{x} \\
\Delta y(t) &=h(x(t), u(t), \delta(t))
\label{y}
\end{align}
where the state $x(t) \in \mathbb{R}^{n}$ with $x(0)=x_{0}$, the measurement output deviations $\Delta y(t) \in \mathbb{R}^{m}$, the control input $u(t) \in \mathbb{R}^{m}$ (e.g., could represent set-points for states regulation), and $\mathcal{N}=$ $\{1, \cdots, n\}$ represents the index set of the ICS components.  $\delta(t) \in \mathbb{R}^{n_{\delta}}$ denotes the piecewise vector of constant %reference 
signals including disturbances, measurement noise, and unknown control parameters. % (e.g., could model set-point changes to other control loops and unmeasured system changes). 
The model in Eqs. \eqref{x}, \eqref{y} may describe water treatment facility, a desalination plant, a microgrid or any other cyber-physical ICS, and might have been derived under suitable regularity constraints from a more general differential-algebraic model \cite{8025384}.  
%The process noise $w_{t} \in \mathbb{R}^{n}$ and the measurement noise $v_{t} \in \mathbb{R}^{m}$ obey some zero-mean stochastic distributions. Moreover, $A \in \mathbb{R}^{n \times n}$ is the system matrix, $B \in \mathbb{R}^{n \times p}$ is the actuator matrix and $C \in \mathbb{R}^{m \times n}$ is the measurement matrix. In the rest of paper, it is assumed that $(A, C)$ is observable and $(A, B)$ is controllable. This condition holds during normal operation of the ICS, even in presence of sensor failures, due to redundancy in measurements.



\subsubsection{Steady state definition in ICS environments}

One major requirement of any CE experiment is to determine the system's steady state, i.e., that state which the performance of the system is contributing towards maintaining a particular system property in a specific pattern or within a specific range. The objective in this part is the model development of the system in such a way to be able to describe the steady states according to the anticipated conditions of the system metrics. In the scenario of ICS, such metrics could be the level of Sodium Hydroxide in a water treatment plant \cite{oxfordus}.


\begin{definition}[Steady State Stability and Synchronization]\label{def:steadystatestability} There exist domains $\mathcal{V} \subseteq \mathbb{R}^{m} \times \mathbb{R}^{n_{\delta}}$ and $\mathcal{W} \subseteq \mathbb{R}^{n}$ for which:  

(1) $g$ and $h$ are Lipschitz continuous functions on $\mathcal{W} \times \mathcal{V}$,



(2) A Lipschitz continuous function $\phi_{w}$ on $\mathcal{W}$ is differentiable $\phi_{w}: \mathcal{V} \rightarrow \mathcal{W}$ and  $\forall (u, \delta) \in \mathcal{V}$ satisfies $0=g\left(\phi_{w}(u, \delta), u, \delta\right)$, i.e.,  each pair $(u, \delta) \in \mathcal{V}$ is unique on $\mathcal{W}$'s equilibrium state $\phi_{w}(u, \delta)$.

(3) There exist constants $c_{j}>0$, $j \in \mathbb{N}: j \in[1, 4]$, and a continuously differentiable function $f$ in $(x, u)$, $ f: \mathcal{W} \times \mathcal{V} \rightarrow \mathbb{R}_{\geq 0}, \quad(x,(u, \delta)) \mapsto f(x, u, \delta)$ for which $ \forall x \in \mathcal{W}$ and $ \forall (u, \delta) \in \mathcal{V}$: 
$$
\begin{array}{c}
c_{1}\left\|x-\phi_{w}(u, \delta)\right\|_{2}^{2} \leq f(x, u, w) \leq c_{2}\left\|x-\phi_{w}(u, \delta)\right\|_{2}^{2} \\
\nabla_{x} f(x, u, w)^{\top} f(x, u, \delta) \leq-c_{3}\left\|x-\phi_{w}(u, \delta)\right\|_{2}^{2} \\
\left\|\nabla_{u} f(x, u, \delta)\right\|_{2}<c_{4}\left\|x-\phi_{w}(u, \delta)\right\|_{2}
\end{array}
$$

%\hl{harrys: explain more about norms + constants}

\noindent (1)-(3) essentially present a singular perturbation problem in which relaxations and other variants exist, and (3) in particular, is a Lyapunov function determining exponential stability of  $\phi_{w}(u, \delta) \in \mathcal{W}$ \cite{phat2007exponential}.

(4) the input-to-output equilibrium mapping $\Delta \bar{y}(u, \delta)=h\left(\phi_{w}(u, \delta), u, w\right): \mathcal{V} \rightarrow \mathbb{R}^{m}$  has the form of:
\begin{align}
\begin{split}
 \Delta \bar{y}(u, \delta)&=h\left(\phi_{w}(u, \delta), u, w\right)\\
 =&({1}/{\gamma})* \mathbbm{1}_{m}*\left(\mathbbm{1}_{m}^{\top} \bar{u}-d\right)   
 \label{equlibrium}
\end{split}
\end{align}
where $\gamma>0$, $\mathbbm{1}_{m}$ representing the indicator function of size $m$, and $d_{cu} \in \mathbb{R}$ is an unmeasured constant disturbance.

\noindent  (4) shows that in steady state conditions, the synchronization of output measurements is possible with deviations being the same at all ICS components. The steady state of an output state can be seen as $\mathbbm{1}_{m}^{\top} u-d$, e.g., the difference of load demand and generation control inputs in a power grid model. The linear span of the indicator function is chosen due to the objective of having finite linear combinations as indicator step functions on arbitrary intervals. 
%\hl{G: ``we take the linear span of the indicator function because we only want finite linear combinations as indicator step functions on arbitrary intervals''}
\end{definition}


In ICS, system operators or automated functionalities of the ICS allocate actions to the actuating elements of the systems in an effort to operate across nominal system setpoint metrics. The target setpoints can be determined in a minimization-type of problem:
\begin{align}
\begin{array}{cl}
\underset{{u}_{h} \in \mathbb{R}^{2}}{\operatorname{minimize}} & z({u}_{h}):=\sum_{j \in  \mathrm{V}} z_{j}\left({u}_{h}{_{j}}\right) \\
\text {s.t.} & 0=\mathbbm{1}_{m}^{\top} u-d_{cu}
\end{array}
\label{minimization}
\end{align}
%\hl{G: ``maybe j in sum should be member of N? $\sum_{j \in \mathcal{N}}$'} \\
where $j \in  \mathrm{V}$ and $|\mathrm{V}| = m$ is the set of the system nodes. Eq. \eqref{minimization} is assumed to be strictly feasible, i.e. the constraint is satisfied. $z_{j}: \mathcal{U}_{i} \rightarrow \mathbb{R}$ models the disutility of the $j_{\text{th}}$ ICS component of not satisfying system nominal demands, and encompasses a barrier function to enforce inequalities ${u}_{{h}_{j}} \in \mathcal{U}_{j}=\left({u}_{{l}_{j}}, {u}_{{h}_{j}}\right),$
where $-\infty \leq {u}_{{l}_{j}}<{u}_{{h}_{j}} \leq+\infty$.   The constraint of Eq. \eqref{minimization} ensures balance of system control inputs $\mathbbm{1}_{m}^{\mathrm{T}} u$ and unmeasured distrubances $d_{cu}$. In addition, by Eq.  \eqref{equlibrium}, Eq. \eqref{minimization} ensures that the steady state system deviations should lead to zero. An example metric following the last minimization problem could be defined as the frequency regulation setpoint of secondary frequency control of ICS in power grids. 

\subsubsection{Formulating hypotheses}

Once the metrics are determined and the steady state behavior of the ICS is understood, the experimental hypotheses can be defined. The objective is to determine what is expected as the result of an experiment, in terms of the system's steady state conditions, if we apply a set of diverse events into the ICS. Lemma \ref{distributedoptimalityconditions} relies on the minimization problem of Eq. \eqref{minimization} to determine under some assumptions the outcome of the experiment in terms of the target setpoints.

\begin{definition}[Direct Graph and Connectivity]\label{def:directgraph}
A sensor network of an ICS can be seen as a topological map represented by a directed graph $\mathcal{G}=(\mathrm{V}, \mathrm{E}, \mathrm{A})$ with nodes $\mathrm{V}=\{1, \ldots, m\}$, edges $\mathrm{E} \subseteq \mathrm{V} \times \mathrm{V}$, and $\mathrm{A}=\left[a_{i j}\right] \in \mathbb{R}^{m \times m} $ is a weighted
adjacency matrix with non-negative adjacency elements, i.e., $a_{i j} \geq 0$, and $a_{i j}>0~\text{if and only if the edge}~(i, j) \in \mathrm{E}$. The neighbors of node $i$ are defined as $\mathcal{N}_{i} \triangleq\{j \in \mathrm{V}:(i, j) \in \mathrm{E}\}$.
\end{definition}

\begin{definition}[Laplacian Matrix]\label{def:laplacian}
The Laplacian matrix $\mathrm{L} \in \mathbb{R}^{m \times m}$ of the graph $\mathcal{G}$ of Definition \ref{def:directgraph} is defined by its elements given by:
$$
L_{i j}=\left\{\begin{array}{ll}
-a_{i j} & \text { if } i \neq j \\
\sum_{k \neq i} a_{i k} & \text { if } i=j
\end{array}\right.
$$
Every row sum of $\mathrm{L}$ is zero. As for its eigenvalues $\lambda$, by definition there exist $\lambda_j = 0$ with right-eigenvector $\mathrm{X_{R_j}} = \mathbbm{1}_{m}$ and the rest $\lambda_i$, $i \neq j$, have positive real part \cite{7810500}. 
\end{definition}

\begin{definition}[Globally Reachable Node]\label{def:reachablenode}
%A directed path in $\mathcal{G}$ is an ordered sequence of nodes such that any pair of consecutive nodes in the sequence is a directed edge of $\mathcal{G}$. 
A node $v_{i} \in \mathrm{V}$ is a globally reachable node, if there exists a path (i.e. a combination of edges in $\mathrm{E}$) from it to every other nodes in $\mathcal{G}$.  
\end{definition}

The next lemma shows an important property of Laplacian $\mathrm{L}$. 
\begin{lemma}\label{laplacianeigen}
The graph $\mathcal{G}$ has a globally reachable node if and only if the Laplacian $\mathrm{L}$ of $\mathcal{G}$
has a simple zero eigenvalue. In this scenario, the left-eigenvector $\mathrm{X_{L_j}} \in \mathbb{R}^{m}$ of $\mathrm{L}$ associated with the simple $\lambda_j = 0$ is $\mathrm{X_{L_j}} \geq 0$, and $\mathrm{X_{L_j}} >0$ if and only if node $v_{j} \in \mathrm{V}$ is globally reachable.
\end{lemma}

\begin{lemma}\label{distributedoptimalityconditions}
Consider Definition \ref{def:directgraph} of a sensor network of an ICS represented by a weighted directed graph $\mathcal{G}=(\mathrm{V}, \mathrm{E}, \mathrm{A})$ with Laplacian matrix $\mathrm{L}$, and let such graph to follow also Definition \ref{def:reachablenode}, i.e., include a globally reachable node and the left-eigenvector $\mathrm{X_{L_j}} \in \mathbb{R}_{\geq 0}^{m}$ of $\mathrm{L}$ to correspond to its simple eigenvalue $\lambda_j = 0$. Let $\Delta \bar{y}$ follows the form of Eq. \eqref{equlibrium} and ${u}_{h} \in \mathbb{R}^{m}$, then for the case of a diagonal matrix $D \succeq 0$ for which $\mathrm{X_{L_j}}^{\top} D \mathbbm{1}_{m}>0$, there exist the following equivalent statements: 
(1) ${u}_{h}$ is the unique optimal solution of Eq. \eqref{minimization}; and 
(2) the vector $q_h \in \operatorname{span}\left(\mathbbm{1}_{m}\right)$ is unique and satisfies:
\begin{subequations}
\begin{align}
0=D \Delta \bar{y}(u_h, \mathrm{X_{L_j}})+\mathrm{L} q_h \label{5a}\\
{u}_h=\nabla \cdot z^{*}(q_h)\label{5b}
\end{align}
\end{subequations}
where $z^{*}(q)=\sum_{j \in \mathrm{V}} z_{j}^{*}\left(q_{j}\right)$ is the conjugate of $z.$

\end{lemma}

The proofs of Lemma \ref{laplacianeigen} and Lemma \ref{distributedoptimalityconditions} are omitted due to space requirements and can be found in literature
\cite{bullo2009distributed, 7810500}.

The hypotheses in CE experiments are typically in the form of ``the events we are injecting into the system will not cause the system’s behavior to change from steady state'' \cite{rosenthal2017chaos}. Since the target metric setpoints can be determined via the optimization of Eq. \eqref{minimization}, and since according to Lemma \ref{distributedoptimalityconditions}, ${u}_h$ is the unique primal optimizer of Eq. \eqref{minimization}, then we can conclude that such formulation leads to a close-form solution not causing the system behavior to deviate from the steady state conditions. The close-form solution enables the analytical expression with a number of known functions in order to follow the concept of a well-defined steady behavior and hypotheses, in comparison with a problem solved with  a numerical solution which would be only an approximate.


%\hl{expand a little bit more}

\subsubsection{Varying ICS process events}

In any system, and therefore in any ICS, unpredictable events attributed to hardware or software faults/malfunctions, adverse malicious data, extreme operating conditions (e.g., high temperatures), etc. can lead to certain system conditions in which can further lead to system or sub-systems failures. In CE, the goal is to induce real-world events into the ICS which can be controlled. Following the formulation of the previous CE model, we follow the paradigm of linear distributed control or typically termed distributed averaging proportional integral (DAPI) control, often deployed in multi-agent networked systems in order to control system elements towards a consensus objective \cite{7990560}. Under this concept, the system components/agents in the distributed ICS (e.g., PLC devices) exchange information with other agents in order to take the proper control decisions (locally), often using linear PI (proportional integral) controls in an effort to minimize the agents' differences. 
If we consider the $\mathcal{N}$ agents of the ICS  to follow DAPI control, then the control dynamics of $u_{j}(t)$, $j \in \mathcal{N}$, can be represented as follows: 
\begin{equation}\label{dapi}
\dot{u}_{j}(t) =\sum_{\ell \in \mathcal{N}, \ell \neq j} a_{j \ell}\left(x_{\ell}(t)-x_{j}(t)\right)+\beta_{j}(t) 
\end{equation}
\noindent  $a_{i k}$ follows Definition \ref{def:directgraph} and it is a binary index of the unidirectional connectivity: if $a_{i k} = 1$, node $i$ can receive data from $k$, and  if $a_{i k} = 0$ there is no unidirectional communication from $k$ to $i$. $\beta_{j}(t)$ can be seen as the bias term to balance ICS operating set-points.

Let $C$ be a diagonal matrix to include the coefficients of the local measurement $C_{j}$ with $j=\{1, \ldots, n\}$. The differentiation of the local measurement data from other data sent from other system agents (remote) can lead to re-writing Eq. \eqref{dapi} as follows: 
\begin{equation}\label{dapiorganized}
\dot{u}_{j}(t) ={-C_{j} x_{j}(t)}+{\sum_{\ell \in \mathcal{N}, \ell \neq j} a_{j \ell} x_{\ell}(t)}+{\beta_{j}(t)}
\end{equation}
\noindent in which the terms represent the local information, the remote information, and the system bias, respectively. Following Definition \ref{def:directgraph} of the adjacency matrix representing the remote connectivity index of the ICS network, we can organize Eq. \eqref{dapiorganized} as: 
\begin{equation}\label{dapivector}
  \dot{u}(t)=(-C+A) x(t)+\beta(t)=-Q x(t)+\beta(t),  
\end{equation}
\noindent where $Q=C-A$. According to \cite{1333204}, and because  $Q$ is essentially a positive semi-definite matrix with every row sum being zero, the system has a steady-state equilibrium in consensus based on the control updates of Eq. \eqref{dapiorganized} if the ICS network agents form an undirected and connected graph. When $\beta=0$, any system equilibrium is in a consensus: by $x_{j}=x_{i}, j, i \in \mathcal{N}$.


\subsubsection{Run experiments in ICS production \& experiment automation}

A major difference of CE compared to accepted forms of security testing is the automation  within the system's production environment as well as the focus on the overall system behavior. Security automation drives continual supervision of the system, which especially in ICS is required due to continuous system changes, e.g., valves pressure, poisoning data, etc. We cannot be aware \textit{a priori} which conditions to the production environment will change the results of a CE test. In this experimentation stage, ideally, the tests need to be tested on the production environment. However, if that is not possible, experiments must be examined in testing conditions as close as possible to the production environment in order to reduce risks in terms of experiments validity  increased reliability, and provide enhanced insight into the performance of the experiments in terms of results confidence.  


\subsubsection{Minimize the Blast Radius}

CE experiments should contribute in minimizing the blast radius of adverse events to the overall system operation, i.e., limit the range and severity of injected events to the system. A resilient ICS resulted from the CE experiments should reduce to the maximum the effects of adverse events. Such events, via the continuous CE experimentation, could be fully characterized providing full understanding of the initial conditions that drove them. Thus, it is of paramount importance to develop probabilistic models for asset availability, accessibility, and usability during and succeeding a major event. The task is complex and is dependent on multiple, interacting and often counterintuitive correlations between variables. 

==> 5-conclusions.tex <==
\section{Conclusions and Future Work}

In this paper, we adopt the concept of CE and present how it can be utilized for complex CPS, and specifically, ICS environments in which adverse events can affect the operating system states. We have examined the related work in the area and set up a formal CE model of nonlinear ICS that generalizes over the CE experimentation steps. We have also described a use-case scenario based on the TEC chemical process. In our future work, we aim to develop a resilience assessment framework in a methodological approach that will utilize the concept of CE to quantify the resilience of industrial CPS. The goal is not only to expand the theoretical and experimentation contribution of this work, but also develop automated restoration policies against classes of adverse events which can be utilized in practical systems. Furthermore, we plan to identify necessary and sufficient conditions which can ensure steady state system operation under stealthy cyber-attacks and evaluate them in a realistic HIL testbed. 
